Enhancing Instruction-Following Capability of Visual-Language Models by Reducing Image Redundancy

Large Language Models (LLMs) have strong instruction-following capability to interpret and execute tasks as directed by human commands. Multimodal Large Language Models (MLLMs) have inferior instruction-following ability compared to LLMs. However, there is a significant gap in the instruction-following capabilities between the MLLMs and LLMs. In this study, we conduct a pilot experiment, which demonstrates that spatially down-sampling visual tokens significantly enhances the instruction-following capability of MLLMs. This is attributed to the substantial redundancy in visual modality. However, this intuitive method severely impairs the MLLM's multimodal understanding capability. In this paper, we propose Visual-Modality Token Compression (VMTC) and Cross-Modality Attention Inhibition (CMAI) strategies to alleviate this gap between MLLMs and LLMs by inhibiting the influence of irrelevant visual tokens during content generation, increasing the instruction-following ability of the MLLMs while retaining their multimodal understanding capacity. In VMTC module, the primary tokens are retained and the redundant tokens are condensed by token clustering and merging. In CMAI process, we aggregate text-to-image attentions by text-to-text attentions to obtain a text-to-image focus score. Attention inhibition is performed on the text-image token pairs with low scores. Our comprehensive experiments over instruction-following capabilities and VQA-V2, GQA, TextVQA, MME and MMBench five benchmarks, demonstrate that proposed strategy significantly enhances the instruction following capability of MLLMs while preserving the ability to understand and process multimodal inputs.

==> sec/tabs/tasks_description.tex <==
\begin{table*}[htbp]
\centering
\caption{Categorization of Multimodal Model Tasks}
\begin{tabular}{l | l | l}
\hline
\textbf{Category} & \textbf{Tasks} & \textbf{Description and Unified Introduction} \\
\hline
Text Formatting & Remove Commas, Lowercase Conversion, Uppercase Conversion & Text formatting tasks standardize textual presentation through punctuation adjustment and case conversion. \\
\hline
Content Detection & Bullet Points Detection, Placeholder Detection, Postscript Detection & Content detection tasks focus on identifying specific elements like bullet points, placeholders, and postscripts within texts. \\
\hline
Format Detection & Highlight Detection, JSON Format Detection, Section Format Detection, Title Format Detection & Format detection tasks ensure accurate identification and handling of structured formats like JSON and highlighted sections. \\
\hline
Task Constraints & Sentence Length Limit, Word Count Limit & Constraint tasks manage the length of content, focusing on sentence and word count limitations for concise communication. \\
\hline
Keyword and Structure Management & Dual Response Combination, Ending Constraint, Keyword Inclusion, Starting Constraint & Keyword and structure management tasks tailor content to start or end in specific ways and integrate essential keywords for targeted relevance. \\
\hline
\end{tabular}
\end{table*}

For evaluation of the model's instruction-following capabilities, we require the LMM to perform the following 15 different verifiable instruction-following tasks. And we divide them into 5 categories:
\begin{itemize}
    \item Text formatting: Remove Commas(T1), Lowercase Conversion(T2), Uppercase Conversion(T3).
    \item Including required content: Placeholder(T4), Postscript(T5), Title(T6), Keyword(T7)
    \item Specific format: Adding Highlights(T8), JSON Format(T9), Answering in Sections(T10), Answer in Bullet Points(T11).
    \item Length: Sentence Length Limit(T12), Word Count Limit(T13).
    \item Other: Dual Response Combination(T14), Ending Constraint(T15), Starting Constraint(T16)
    
\end{itemize}
